Mars Image Content Classification: Three Years of NASA Deployment and Recent Advances

The NASA Planetary Data System hosts millions of images acquired from the planet Mars. To help users quickly find images of interest, we have developed and deployed content-based classification and search capabilities for Mars orbital and surface images. The deployed systems are publicly accessible using the PDS Image Atlas. We describe the process of training, evaluating, calibrating, and deploying updates to two CNN classifiers for images collected by Mars missions. We also report on three years of deployment including usage statistics, lessons learned, and plans for the future.

==> Makefile <==
DOC = pds-classifier-21
CLEAN = *.log *.aux *.out *.bbl *.blg *.acr *.acn *.glg *.gls *.glo *.ist *.alg *.cut
CLEANER = *.pdf

all:
	pdflatex $(DOC)
	if grep -c -q '\\citation' $(DOC).aux; then bibtex $(DOC); fi
	pdflatex $(DOC)
	pdflatex $(DOC)

zip:
	cd .. ; zip pds-21-iaai.zip 21-iaai-pds-classifier/{*tex,*sty,*bib,*bst,Makefile} 21-iaai-pds-classifier/figures/{PSP_002912_2075_RED-crater.png,usage/MRO_queries.pdf,usage/MSL_queries.pdf,hirise_dist.pdf} 21-iaai-pds-classifier/figures/hirise/{brightdune.png,crater.png,darkdune.png,ejecta.png,other.png,streak.png,spider.png,swiss.png,cm-test-matrix.pdf,ece_with_cal_matrix-crop.pdf,pr-test-hirise.pdf,validation_set_spiders_2.png,test_set_spiders_2.png} 21-iaai-pds-classifier/figures/{msl*jpg,mslnet-reliability-diagram-crop.pdf,mslnet-pr.pdf} ; cd -

clean:
	rm -f $(CLEAN)

cleaner: clean
	rm -f $(CLEANER)


==> pc21-mer-dataset.tex <==
\subsection{MER Surface Data Set}

The \ac{MER} surface data set consists of \num{68602} images collected by the
\ac{Pancam} instruments mounted on both Spirit and Opportunity rovers. They each
have a \ac{Pancam} instrument mounted on the rover mast. \ac{Pancam} is a
two-instruments suite consisting of a left eye camera and a right eye camera.
The \ac{Pancam} was primarily used to image Mars surface and sky for science
analysis. Each \ac{Pancam} camera has 8 filters, with wavelengths ranging from
400 \si{nm} to \num{1100} \si{nm}, which provide color imaging capability.  

As a first step of \ac{MER} surface data set creation, we discovered \num{24}
distinct classes based on the results of a survey conducted by the MER Data
Catalog project, in which scientists and engineers who worked on \ac{MER}
mission were asked, among other things, about the types of objects or phenomena
they had interest in searching for in \ac{MER} data. In addition, we used
DEMUD~\cite{wagstaff:demud13}, a diversity-based novelty detection algorithm, to
rank a subset of images to make the class discover process more efficient. As
the results of class discovery, the following \num{24} classes belonging to 5
conceptual groups were identified, and example of each class is shown in
Figure~\ref{fig:mer-ds}. The examples are images taken by the L2 filter of the
\ac{Pancam} cameras of both rovers. 

\begin{itemize}
\item Rover hardware group: rover deck, pancam calibration target, rover arm,
	other hardware
\item Artificial geology group: rover tracks, soil trench, RAT brushed target, 
	RAT hole
\item Natural geology group: outcrop rock, float rock, clasts, bright soil, 
	dunes/ripples, rock (linear features), rock (rounded features), soil,
	spherules
\item Image type group: distant vista, sky, close-up rock, nearby surface,
	rover parts
\item Miscellaneous group: astronomy, artifacts
\end{itemize}

The \ac{MER} mission completed on February 13, 2019 due to a historical dust
storm on Mars in June, which means there will not be new \ac{Pancam} images
added to the \ac{MER} mission data archive. For that reason, we employed a
spatial sampling strategy for the creation of the \ac{MER} surface data set.  We
randomly sampled 20\% of images from each site location, and this resulted in a
data set of \num{3004} images. We then utilized Zooniverse (\todo{cite}) to
label these images. The \ac{Pancam} images often contain more than one object of
interest, so we allowed multiple labels to be assigned to each image.  The class
distribution of the \ac{MER} surface data set is shown in
table~\ref{tab:mer-class-distribution}. We split these images into training,
validation, and test sets by the location of acquisition to ensure that images
taken from the same location appear in only one set. We used rougly 60\% of the
images for training, 15\% for validation, and 25\% for testing. This resulted in
\num{1806} training images, \num{456} validation images, and \num{742} test
images. The training and validation images were augmented using rotation,
skewing, and shearing methods with different parameter values. Since each
transformation is followed by a square crop to keep the image size consistent,
we constrained the limits of parameter values of each augmentation method to
avoid cropping out important features at the edges of images. For each source
image, we created 29 augmented images. This resulted in \num{54180} training
images and \num{13680} validation images.

\begin{center}
\begin{tabular}{|c|c|c|} \hline
\bf Class Name & \bf Count & \bf \% of data set \\ \hline
Rover deck & \num{222} & 7.39\%  \\ \hline
Pancam cal. target & \num{14} & 0.47\%  \\ \hline
Rover arm & \num{4} & 0.13\%  \\ \hline
Other hardware & \num{116} & 3.86\%  \\ \hline
Rover tracks & \num{301} & 10.02\%  \\ \hline
Soil trench & \num{34} & 1.13\%  \\ \hline
RAT brushed target & \num{17} & 0.57\%  \\ \hline
RAT hole & \num{30} & 1.00\%  \\ \hline
Outcrop rock & \num{1915} & 63.75\%  \\ \hline
Float rock & \num{860} & 28.63\%  \\ \hline
Clasts & \num{1676} & 55.79\%  \\ \hline
Bright soil & \num{122} & 4.06\%  \\ \hline
Dunes/ripples & \num{1000} & 33.29\%  \\ \hline
Rock (linear features) & \num{943} & 31.39\%  \\ \hline
Rock (rounded features) & \num{219} & 7.29\%  \\ \hline
Soil & \num{2891} & 96.24\%  \\ \hline
Astronomy & \num{12} & 0.4\%  \\ \hline 
Spherules & \num{868} & 28.89\%  \\ \hline
Distant vista & \num{903} & 30.23\%  \\ \hline
Sky & \num{954} & 31.76\%  \\ \hline
Close-up rock & \num{23} & 0.77\%  \\ \hline
Nearby surface & \num{2006} & 66.78\%  \\ \hline
Rover parts & \num{301} & 10.02\%  \\ \hline
Artifacts & \num{28} & 0.93\%  \\ \hline
\end{tabular}
\captionof{table}{The class distribution of the \ac{MER} surface data set.
	Multiple labels are allowed to be assigned to each image, so the
	percentages do not sum to 100\%}
\label{tab:mer-class-distribution}
\end{center}


\begin{figure*}
% First row
\subfigure[Artifacts]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-artifacts.jpg}}
\subfigure[Astronomy]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-astronomy.jpg}}
\subfigure[Bright soil]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-bright-soil.jpg}}
\subfigure[Clasts]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-clasts.jpg}}
\subfigure[Close-up rock]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-closeup-rock.jpg}}
\subfigure[Distant vista]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-distant-vista.jpg}}
% Second row
\subfigure[Dunes/ripples]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-dunes-ripples.jpg}}
\subfigure[Float rock]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-float-rocks.jpg}}
\subfigure[Nearby surface]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-nearby-surface.jpg}}
\subfigure[Other hardware]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-other-hardware.jpg}}
\subfigure[Outcrop rock]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-outcrop-rock.jpg}}
\subfigure[Pancam cal. target]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-pancam-cal-target.jpg}}
% Third row
\subfigure[RAT brushed target]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rat-brushed-target.jpg}}
\subfigure[RAT hole]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rat-hole.jpg}}
\subfigure[Rock (linear features)]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rock-linear.jpg}}
\subfigure[Rock (rounded features)]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rock-rounded.jpg}}
\subfigure[Rover arm]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rover-arm.jpg}}
\subfigure[Rover deck]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rover-deck.jpg}}
% Fourth row
\subfigure[Rover parts]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rover-parts.jpg}}
\subfigure[Rover tracks]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-rover-tracks.jpg}}
\subfigure[Sky]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-sky.jpg}}
\subfigure[Soil trench]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-soil-trench.jpg}}
\subfigure[Soil]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-soil.jpg}}
\subfigure[Spherules]
{\includegraphics[width=0.16\textwidth]{figures/mer-ds-spherules.jpg}}
\caption{Example image of each class in \ac{MER} surface data set.}
\label{fig:mer-ds}
\end{figure*}


==> pc21-mernet-eval.tex <==
\subsection{MERNet Evaluation (Steven)}


==> pc21-mernet.tex <==
\subsection{MERNet (Steven)}
\begin{itemize}
\item baseline approach - 25 binary classifiers
\item classifier chain
\item interpretability - prototypes (MOVE TO Future Work)
\end{itemize}

MERNet refers to a content-based image classification pipeline deployed for the
\ac{MER} \ac{Pancam} images hosted by the NASA \ac{PDS} \ac{Imaging Node}.
Unlike HiRISENet and MSLNet, MERNet was built with multi-label capability, which
allows multiple labels to be assigned to a single image. The advantage of
building a multi-label classification system is that it no longer requries an
image to be described by the class of the dominant feature, instead, the image
can be described by all classes presented. 

We employed transfer learning techniques with three \ac{CNN} architectures
to adapt weights trained using Earth images to Mars images. For the first
approach, we transformed the multi-label classification problem into N
independent one-verse-all binary problems, where N is the total number of 
classes and in this case N equals twenty-four. The feature outputs were pooled
through a fully connected layer, and then an element-wise sigmoid function was
used to convert the logit vectors into posterior probabilities. To train this
\ac{CNN} classifier, we minimized the mean binary cross-entropy loss across each
class using stochastic gradient descent. The loss function can be expressed, for
a batch of size $n$, label target $y$, and output prediction scores $\hat{p}$,
as the functional form in (\ref{eqn:mcel}). 

\begin{equation} \label{eqn:mcel}
    L_{\text{batch}} = -\frac{1}{24n}\sum_{i=1}^n\sum_{j=1}^{24} y_j\log(\hat{p}_j) + (1-y_j)log(1-\hat{p}_j)
\end{equation}

For the second \ac{CNN} architecture, we employed the classifier chain
methodology in \todo{cite classifier chain paper}. The classifier chain method
modifies the fully connected layer by instead calculating logit vectors one at a
time, then iteratively appending them to the input for successive logit
calculations. This approach allows for the \ac{CNN} classifier to lean
dependencies between certain classes, analogous to expressing a conditional
probability with available class information rather than treating each class as
completely independent. In addition, the image site location was also encoded as
a feature and appended to the logit vectors. The motivation behind this was that
the network could leverage a learned distribution of classes within each site
location to more informed decisions about the label predictions. In order to
fully leverage this chain structure, general image information such as image
type was placed at the front of the classifier chain, while more fine-grained
categories such as natrual geology were placed near the end of the chain. The
exact order of the class category groupings was image type, followed by rover
parts, artificial geology, then natural geology. 

